Evaluation of Legged Robot Landing Capability Under Aggressive Linear and Angular Velocities

This paper proposes a method to evaluate the capability of aggressive legged robot landing under significant touchdown linear and angular velocities upon impact. Our approach builds upon the Planar Inverted Pendulum with Flywheel (PIPF) model and introduces a landing framework for the first stance step on a non-dimensional basis. We develop a nonlinear framework with iterative constrained trajectory optimization to stabilize the first stance step prior to N-step Capturability analysis. Performance maps across many different initial conditions reveal approximately linear boundaries as well as the effect of inertia, body incidence angle and leg attacking angle on the boundary shape. Our method also yields the engineering insight that body inertia affects the performance map the most, hence its optimization can be prioritized when the target is to improve robot landing efficacy.

==> Others/ideas.tex <==
Questions that should be answered in this paper:

How to determine the number of steps needed to finish a landing motion? 
From the energy perspective, it is about how much energy the system can dissipate during each step.

Is the actuated pitch-involved SLIP (APSLIP) sufficient for regulating landing motion? 
In other words, what is the boundary of its attraction basin in terms of landing translational/rotational energy/momentum?
Is heavy-tail-SLIP a better model with larger attraction basin?

Why MPC is not suitable for this scenario? Or could we apply MPC on this hybrid system (with unknown switching time instance)?
If it is feasible, we could make use of it to produce some kind of baseline for performance evaluation.

Could we decouple rotational states (pitch) from translational states (x, z) so that we can stabilize each group in separate steps (and may even predict number of steps required).

Concepts:

Capture state = the state with zero kinetic energy level
Capture region = set of Capture points
Capture point method: placing foot on a Capture point = move states to Capture state
Q: Is it feasible with large angular momentum? Is SLIP compatible? (IP and LIP are compatible.)
A: Here is the thought. SLIP may not even a suitable template from the very beginning. It is intended to store and reuse the kinematic energy to maintain the energy level, while landing requires more of an absorbor. It could be better to focus on LIP as leg model and investigate which kind of energy the elastic spine could help absorbing (maybe is also related to [spring storage capacity / angular kinematic energy] and some other parameters) as well as how to design the attacking angle.

From the observation of Bobcat landing during a standing long jump, the spine and fore leg are almost co-linear. It could be a starting point for investigating the proper region of the attacking angle.

==> Others/tech_log.tex <==
12/31/2021
In optimal control, there are many factors of interest in the solver setup. To have a relatively fair comparison, I choose the same time step (0.002s) for all tests.

Cost function: End point cost
Impact factor: weights / control horizon
Best case so far: 
    control horizon = TC/3, k = [1 1e4 1e2 1e2] >> both xdot and zdot head to 0, both gamma and gammadot converge to 0
    control horizon = TC/5, k = [1 1e2 1e2 1e2] >> both xdot and zdot head to 0, both gamma and gammadot converge to 0
Observation: This cost function is sensitive to ( control horizon + weights) 

Cost function: Discounted running cost (discounts fit in Poisson distribution [lambda = 1])
Impact factor: weights / control horizon
Best case so far:
    various weights and horizons >>  both xdot and zdot head to 0, both gamma and gammadot converge to 0
Observation: computing on full history can be less time efficient with longer horizon. A truncated version (taking the last 5 coefficients) provides with almost the same results with faster computation.

01/03/2022
MPC frame work: typical MPC controllers work on either determined long horizon or iterate on determined short horizons. In the stance phase, the exact duration is unknown. Our approach is to 1) approximate the overall stance duration with TC, 2) segment TC into shorter episodes, 3) iterate a MPC over the episodes.

About termination condition, ...

Necessity of adopting different cost types and weights: when the rotation is enforced at the desired position, it should be remain around the destination.

In the first stance phase:

Parameters: m = 80 kg, I = 0.32 kg*m*m
Cost setup: iter=1 -> k = [1 1e4 1e2 1e2]; iter>1 -> k = [1 1e4 1e0 1e0]
v0[dimless] = 1, w0[dimless] = 1 ~ 10, gamma can be stabilized around 0 deg
v0[dimless] = 2, w0[dimless] = 1, gamma cannot be stabilized

Parameters: m = 80 kg, I = 3.2 kg*m*m
Cost setup: iter=1 -> k = [1 1e4 1e2 1e2]; iter>1 -> k = [1 1e4 1e0 1e0]
v0[dimless] = 1, w0[dimless] = 1 ~ 3, gamma can be stabilized around 0 deg
v0[dimless] = 1, w0[dimless] = 4, gamma cannot be stabilized around 0 deg
v0[dimless] = 2, w0[dimless] = 1, gamma cannot be stabilized

01/05/2022
Q: Why we should look into various cost types? 
A: In a stance phase, the model could experience different sub-phases where some states may already be stabilized and the others may not. To those stabilized, we need to focus on maintaining their stability ( which suggests full-horizon control, like uniform cost); to those remaining to stabilize, we should focus on their states converging to the desired equilibrium points ( which suggests partial-horizon control, like end point cost or discounted running cost ).
All costs that should be taken into consideration (all in dimensionless):
1. End point states -> Mayer term
2. Running states, full/truncated history, discounted (Poisson, Geometric, uniform, Beta-binomial) -> Lagrangian term

01/10/2022
Because there is a need to switch between truncated and full history of each state, we need to compute all states of full history and truncate them as needed. This will increase some tolerable amount of execution time comparing to computing all states of truncated history, and we should live with that.
When gamma and gammadot are close to 0, uniform cost of full history does better job in maintaining the the stability than other cost.

01/12/2022
We should try 2 different iteration paradigms:
1) a typical trajectory optimization for each iteration, that is, the prediction horizon equals to the control horizon. Then we should compare 1a) keeping only the first a few steps as the solution and 1b) keeping all steps as the solution.
2) a typical MPC problem for each iteration, that is, the prediction horizon is larger than the control horizon.

In 1b), shorter prediction horizon (e.g., 0.1TC) does not improve the smoothness of the solution. The sudden dropping edge still appears in the end of each iteration. On the other hand, optimal solutions appear to be easier to find for each iteration.
In 1a), 

01/14/2022
After mid-point, gamma and gammadot can still be stabilized and zdot can still be attracted to zero, except xdot will inevitably increase (thus need to justify why this is something we do not want).

01/15/2022
We need to carefully discuss when to terminate the iMPC: how to determine failure conditions or successful conditions?

To complete the whole stance phase, either zdot should be non-negative (not really) or r extends back to r0.

A sufficient condition would be: at the mid-point, zdot >= 0, and pitch static (gamma = 0, gammadot = 0). But it would be very strict. However, after mid-point, pitch dynamics is still likely to be stabilized as long as it is before the inevitable falling down. Then, how to define conditions for the inevitable falling down? 
In other words, 1) if pitch dynamics cannot be stabilized before the first stance phase completes, it fails; 2) if pitch dynamics can be stabilized but the remaining translational kinematic energy (Ek2) cannot be dissipated in the second step, it fails; 3) otherwise, it succeeds.
First stance phase completion conditions: 1) r >= r0; or 2) alpha >= pi; or 3) pitch dynamics stabilized.
Second stance phase feasibility conditions: 1) Ek2 < (Fmax*l0) (necessary)
Note: do not use inverted pendulum in the second phase because the initial contact can exert very large force that may be destructible.

Start to think about the paper title: towards benchmark of athletic landing capability of legged robots? Dimensionless analysis regarding to the athletic landing capability of legged robots?


